Trillium: Higher-Order Concurrent and Distributed Separation Logic for Intensional Refinement

Expressive state-of-the-art separation logics rely on step-indexing to model semantically complex features and to support modular reasoning about imperative higher-order concurrent and distributed programs. Step-indexing comes, however, with an inherent cost: it restricts the adequacy theorem of program logics to a fairly simple class of safety properties. In this paper, we explore if and how intensional refinement is a viable methodology for strengthening higher-order concurrent (and distributed) separation logic to prove non-trivial safety and liveness properties. Specifically, we introduce Trillium, a language-agnostic separation logic framework for showing intensional refinement relations between traces of a program and a model. We instantiate Trillium with a concurrent language and develop Fairis, a concurrent separation logic, that we use to show liveness properties of concurrent programs under fair scheduling assumptions through a fair liveness-preserving refinement of a model. We also instantiate Trillium with a distributed language and obtain an extension of Aneris, a distributed separation logic, which we use to show refinement relations between distributed systems and TLA+ models.

==> lstcoq.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{coq} {
% Comments may or not include Latex commands
texcl=false,

% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Add, Morphism, Relation,
Implicit, Arguments, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Context, Class, Global, Instance, Program, Infix,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Extern, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside, Eval,
Check},

% Gallina
morekeywords=[2]{match, with, end, if, then, else, let, fst, snd},
%morekeywords=[2]{forall, exists, exists2, fun, fix, cofix,
%      match, with, end, as, in, return, let, is, if, then, else,
%      for, of, nosimpl},

% Sorts
morekeywords=[3]{Set, Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
%morekeywords=[4]{
%         pose, set, move, case, elim, apply, clear,
%            hnf, intro, intros, generalize, rename, pattern, after,
%	    destruct, induction, using, refine, inversion, injection,
%         rewrite, congr, unlock, compute, field, fourier,
%            replace, fold, unfold, change, cutrewrite, simpl,
%         have, suff, wlog, suffices, without, loss, nat_norm,
%            assert, cut, trivial, revert, bool_congr, nat_congr,
%	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
%morekeywords=[5]{
%         by, done, exact, tauto, romega, omega,
%         assumption, solve, contradiction, discriminate},


% Control
%morekeywords=[6]{do, last, first, try, idtac, repeat},

morestring=[b]{"},

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% Size of tabulations
tabsize=3,							

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style for listings
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,							

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{red}},
keywordstyle=[2]{\ttfamily\color{blue}},
keywordstyle=[3]{\ttfamily},

%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\ttfamily,

moredelim=[is][\color{black}]{@@}{@},
}

